J/$\psi$ production as a function of charged-particle multiplicity in p-Pb collisions at $\sqrt{\textit{s}_{\rm NN}}~=~8.16$ TeV

Inclusive J/$\psi$ yields and average transverse momenta in p-Pb collisions at a center-of-mass energy per nucleon pair $\sqrt{s_{\rm NN}}$ = 8.16 TeV are measured as a function of the charged-particle pseudorapidity density with ALICE. The J/$\psi$ mesons are reconstructed at forward $(2.03 < y_{\rm cms} < 3.53)$ and backward ($-4.46 < y_{\rm cms} < -2.96$) center-of-mass rapidity in their dimuon decay channel while the charged-particle pseudorapidity density is measured around midrapidity. The J/$\psi$ yields at forward and backward rapidity normalized to their respective average values increase with the normalized charged-particle pseudorapidity density, the former showing a weaker increase than the latter. The normalized average transverse momenta at forward and backward rapidity manifest a steady increase from low to high charged-particle pseudorapidity density with a saturation beyond the average value.

==> table_multiplicity.tex <==
%
%\begin{table}[!htbp]
%   \centering
%   \begin{tabular}{@{} ccc @{}} % Column formatting, @{} suppresses leading/trailing space
%%      \multicolumn{2}{c}{Item} \\
%	\hline
%	$\Ntrc$	 & 		$\dndeta$			&		$\sigma/\sigma_{\rm MB}$ \\ \hline
%	[xx,xx]	&		$xx \pm xx$		&		xx\%
%	\\ \hline
%   \end{tabular}
%   \caption{
%   \label{tab:multiplicity}
%   }
%\end{table}

\begin{table}[!htbp]
   \centering
      \caption{
   \label{tab:multiplicity}
   Charged-particle pseudorapidity density intervals considered and the fraction of visible cross section ($\sigma/\sigma_{\rm MB}$) scrutinised. The values refer to non-single diffractive events. The shown uncertainty is systematic.
   }
   \begin{tabular}{@{} cc|cc @{}} % Column formatting, @{} suppresses leading/trailing space
	\hline
	 \multicolumn{2}{c|}{$2.03 < \ycms < 3.53$} &  \multicolumn{2}{c}{$-4.46 < \ycms < -2.96$}  \\
	$\left( \dndeta \right) /\avdndeta$			&		$\sigma/\sigma_{\rm MB}$ 	&	$\left( \dndeta \right) /\avdndeta$			&		$\sigma/\sigma_{\rm MB}$ 	 \\ \hline
	$0.18 \pm 0.02$	&    0.20 		&	$0.19 \pm 0.02$	&	0.22	\\
	$0.42 \pm 0.03$	&    0.10  		&	$0.47 \pm 0.03$	&	0.12 \\
	$0.58 \pm 0.03$	&    0.07  		&	$0.66 \pm 0.04$	&	0.08 \\
	$0.70 \pm 0.04$	&    0.06 	 	&	$0.80 \pm 0.04$	&	0.06 \\
	$0.82 \pm 0.05$	&    0.06  		&	$0.93 \pm 0.05$	&	0.07 \\
	$0.94 \pm 0.05$	&    0.06  		&	$1.07 \pm 0.06$	&	0.05 \\
	$1.06 \pm 0.06$	&    0.05  		&	$1.21 \pm 0.06$	&	0.06 \\
	$1.18 \pm 0.06$	&    0.05  		&	$1.36 \pm 0.07$	&	0.05 \\
	$1.30 \pm 0.07$	&    0.05  		&	$1.49 \pm 0.08$	&	0.04 \\
	$1.42 \pm 0.07$	&    0.04  		&	$1.63 \pm 0.09$	&	0.04 \\
	$1.54 \pm 0.08$	&    0.04 	 	&	$1.76 \pm 0.10$	&	0.03 \\
	$1.66 \pm 0.09$	&    0.03  		&	$1.89 \pm 0.10$	&	0.03 \\
	$1.78 \pm 0.10$	&    0.03  		&	$2.04 \pm 0.11$	&	0.03 \\
	$1.90 \pm 0.10$	&    0.03  		&	$2.18 \pm 0.12$	&	0.02 \\
	$2.03 \pm 0.11$	&    0.03  		&	$2.32 \pm 0.13$	&	0.02 \\
	$2.22 \pm 0.12$	&    0.03  		&	$2.54 \pm 0.14$	&	0.02 \\
	$2.50 \pm 0.14$	&    0.03  		&	$2.86 \pm 0.17$	&	0.02 \\
	$2.94 \pm 0.17$	&    0.03 	 	&	$3.36 \pm 0.20$	&	0.01 \\
	$3.67 \pm 0.23$	&    0.01  		&	$4.15 \pm 0.28$	&	0.003 \\
	$4.93 \pm 0.36$	&    0.0004 	&	$5.59 \pm 0.44$	&	0.0001 \\	
	\hline
   \end{tabular}
%   \caption{
%   \label{tab:multiplicity}
%   Charged-particle pseudorapidity density intervals considered and the fraction of visible cross section ($\sigma/\sigma_{\rm MB}$) scrutinised. The values refer to non-single diffractive events.
%   }
\end{table}
